The Parallel Semantics Program Dependence Graph

A compiler's intermediate representation (IR) defines a program's execution plan by encoding its instructions and their relative order. Compiler optimizations aim to replace a given execution plan with a semantically-equivalent one that increases the program's performance for the target architecture. Alternative representations of an IR, like the Program Dependence Graph (PDG), aid this process by capturing the minimum set of constraints that semantically-equivalent execution plans must satisfy. Parallel programming like OpenMP extends a sequential execution plan by adding the possibility of running instructions in parallel, creating a parallel execution plan. Recently introduced parallel IRs, like TAPIR, explicitly encode a parallel execution plan. These new IRs finally make it possible for compilers to change the parallel execution plan expressed by programmers to better fit the target parallel architecture. Unfortunately, parallel IRs do not help compilers in identifying the set of parallel execution plans that preserve the original semantics. In other words, we are still lacking an alternative representation of parallel IRs to capture the minimum set of constraints that parallel execution plans must satisfy to be semantically-equivalent. Unfortunately, the PDG is not an ideal candidate for this task as it was designed for sequential code. We propose the Parallel Semantics Program Dependence Graph (PS-PDG) to precisely capture the salient program constraints that all semantically-equivalent parallel execution plans must satisfy. This paper defines the PS-PDG, justifies the necessity of each extension to the PDG, and demonstrates the increased optimization power of the PS-PDG over an existing PDG-based automatic-parallelizing compiler. Compilers can now rely on the PS-PDG to select different parallel execution plans while maintaining the same original semantics.

==> sections/system.tex <==
% System 2 pages 
\label{sec:system_methodology}
The PS-PDG abstraction captures the underlying semantics of a parallel program.
The strength of an abstraction is in its ability to represent knowledge about a program not readily ascertainable from the IR.
The value of a specific abstraction is in what it enables, and it should be evaluated in this way.
To this end, we evaluate the PS-PDG by what it enables for an \emph{existing} automatic-parallelizing compiler rather than the end result of the parallelization.
Notice that evaluating on the end result of a transformation would evaluate the transformation implemented using the PS-PDG, rather than the expressiveness of the PS-PDG itself.
Hence, we performed the following two experiments (further described in the rest of this section) to evaluate the PS-PDG abstraction.
Both experiments are done by enhancing an existing parallelizing compiler making it using the PS-PDG rather than the PDG.
The first experiment measures the expansion to the set of legal parallelization plans that PS-PDG creates.
The second one measures the potential impact of the new parallelization plans that only the PS-PDG has reached.


To perform the two experiments described above, we have implemented a custom compilation pipeline (Figure~\ref{fig:system_pipe}).  
Our pipeline is built upon the NOELLE~\cite{matni2022noelle} compilation framework, which is built upon LLVM~\cite{llvm}.
NOELLE provides an automatic-parallelizing compiler working at the IR level, which supports three loop-based parallelization techniques: DOALL~\cite{doall}, HELIX~\cite{helix}, and DSWP~\cite{dswp}.
We extended this compiler as following.
We added a new front-end that translates OpenMP annotations into \code{pragmas} that make more explicit the semantics of the original OpenMP code.
Then, our custom clang-based front-end generates LLVM IR with custom metadata from it.
This IR with metadata feeds a series of PS-PDG-aware code transformations that are designed to make the code more amenable to parallelization while maintaining the underlying semantics of the parallel program.
Finally, the resulting IR with metadata is used to build the PS-PDG.
The PS-PDG is then used by our extensions of the NOELLE's parallelizing compiler, which originally used the PDG instead.




To understand the potential added by PS-PDG, we enumerate the space of legal parallelization plans that our compiler can consider and we compare it with those that the PDG-based compiler included in NOELLE sees.
We consider the existing options for a loop: parallelization technique, number of cores/chunk size, and minimum required loop hotness.
Additionally, we consider the options now available from undirected edges and/or data-selectors.
We enumerate the space for a 56 physical core machine while only considering loops with at least $10\%$ run-time coverage.
In more detail, if a loop can be parallelized as DOALL (i.e., no loop-carried dependences with number of iterations that will execute known when the loop starts its execution), then we only consider it as DOALL with possible chunk sizes of \code{1,2,4,8}. 
Hence, the number of parallelization plans for this loop is at least 56 (cores) $\times$ 4 (number of chunk sizes considered). 
Parallelization plans for non-DOALL loops are computed adding the possible plans generated by the HELIX execution model to those generated by DSWP's model.
For both models, the subset of the PS-PDG of a given loop is analyzed to identify strongly-connected components (SCC) with loop-carried dependencies.  
For SCCs with loop-carried dependencies, we utilize any PS-PDG features within the SCC to determine if the loop-carried dependencies can be removed (e.g., privatization).  
The SCCs of a loop are then categorized as sequential or parallel accordingly.
For parallelization plans created by HELIX for a loop, we enumerate the possible number of sequential segments of that loop (a sequential segment is a slice of the loop that includes at least one sequential SCC).
We then multiply it by the number of cores that this loop can run on.
Parallelization plans enabled by DSWP are computed by enumerating the number of pipeline stages (a stage includes at least one node of the SCCDAG of the considered loop).

The above evaluation measures the number of legal parallelization plans that PS-PDG makes visible to compilers. 
Next we describe how we have evaluated the goodness of these plans. 
In more detail, to evaluate the potential of the parallelization plans now available to the existing automatic-parallelizing compiler, we measure the critical path of the available parallelism on an ideal machine with unlimited cores, zero cost communication, and perfect memory access.
This enables us to characterize the limit of the additional parallelism unlocked by PS-PDG.
We do so by comparing the limit of the parallelism expressed by programmers, with the one obtainable using PDG, and with the parallelism obtainable using the new PS-PDG abstraction.
In more detail, the critical path is computed as the number of dynamic LLVM instructions that must run sequentially given a parallelization plan.
The PDG measurements assume that every outermost loop is parallelized using DOALL, HELIX or DSWP using the SCCs generated from the PDG.
Lastly, the PS-PDG measurements assume that every outer loop is parallelized using the SCCs from the PS-PDG, as well as inner developer-expressed loops.
We only consider the hierarchical parallelism possible with the existing parallelizing compiler or when developer-expressed.

